Mitigating Backdoor Poisoning Attacks through the Lens of Spurious Correlation

Modern NLP models are often trained over large untrusted datasets, raising the potential for a malicious adversary to compromise model behaviour. For instance, backdoors can be implanted through crafting training instances with a specific textual trigger and a target label. This paper posits that backdoor poisoning attacks exhibit \emph{spurious correlation} between simple text features and classification labels, and accordingly, proposes methods for mitigating spurious correlation as means of defence. Our empirical study reveals that the malicious triggers are highly correlated to their target labels; therefore such correlations are extremely distinguishable compared to those scores of benign features, and can be used to filter out potentially problematic instances. Compared with several existing defences, our defence method significantly reduces attack success rates across backdoor attacks, and in the case of insertion-based attacks, our method provides a near-perfect defence.

==> tab-app-attack.tex <==
\begin{table}[]
    \centering
    \small
    \begin{tabular}{ccrr}
    \toprule
         \textbf{Dataset} &  \makecell{\textbf{Attack}\\\textbf{Method}} & \textbf{ASR}& \textbf{CACC}\\
         \midrule
         \multirow{4}{*}{SST-2} & Benign & --- & 92.4\\
         & BadNet & 100.0 & 92.5\\
         & InsertSent & 100.0 & 91.9\\
         & Syntactic & 95.9 & 92.0\\
         \midrule
         \multirow{4}{*}{OLID} & Benign & --- & 84.0\\
         &BadNet & 99.9 & 84.7\\
         & InsertSent & 100.0 & 83.7\\
         & Syntactic & 99.9	& 83.5\\
         \midrule
       \multirow{4}{*}{AG News} & Benign & ---  &94.6\\
       & BadNet & 99.9 & 94.5\\
         & InsertSent & 99.7 & 94.3\\
         & Syntactic & 99.8 & 94.4\\
         \midrule
        \multirow{4}{*}{QNLI} & Benign & ---  & 91.4 \\
        & BadNet & 100.0 & 91.2\\
         & InsertSent & 100.0 & 91.0\\
         & Syntactic & 99.1 & 89.9\\
    \bottomrule
    \end{tabular}
    \caption{ASR (attack success rate) and CACC (clean test set accuracy) of the benign model and all studied attacks on SST-2, OLID, AG News and QNLI datasets.}
    \label{tab:app_attack}
\end{table}

==> tab-diff-z.tex <==
\begin{table*}
    \centering
    %\scalebox{0.9}{
    \small
    \begin{tabular}{clccccccccc}
    \toprule
        \multirow{2}{*}{\textbf{Dataset}} &  \multirow{2}{*}{\textbf{Defence}} & \multicolumn{3}{c}{\textbf{BadNet}}  & \multicolumn{3}{c}{\textbf{InsertSent}} & \multicolumn{3}{c}{\textbf{Syntactic}}\\
         & & \textbf{BASR} &  \textbf{ASR} & \textbf{CACC} & \textbf{BASR} &  \textbf{ASR} & \textbf{CACC}  & \textbf{BASR} &  \textbf{ASR} & \textbf{CACC} \\
          \midrule
         \multirow{4}{*}{SST2}& None  & --- &100.0& 92.5	&---& 100.0 & 	91.9	&---& \ \ 95.9 & 	92.0\\
         \cmidrule{2-11}
          & \ztoken& \multirow{3}{*}{9.0}  & \quad 9.4 & 92.3 & \multirow{3}{*}{2.9}  &\quad \textbf{3.0} & 92.5 & \multirow{3}{*}{16.9}& \ \ 37.3 & 91.6\\
          & \ztree &  & 100.0  & 92.2 & & \ \ 85.8 & 92.5 & &\ \ 29.7 & 92.1\\
          & \zseq & & \quad \textbf{9.0} & 92.0 & &\quad 3.4 & 92.6 & & \ \ \textbf{29.7} & 92.1\\
         \midrule
         \multirow{4}{*}{OLID} & None & --- & \ \ 99.9 &	84.7 &--- 	&100.0 &	83.7& --- &	\ \ 99.9	& 83.5 \\
         \cmidrule{2-11}
         &\ztoken & \multirow{3}{*}{32.6} & \ \ \textbf{31.5} &	85.0	&\multirow{3}{*}{38.5} &  \ \ 37.6 &	84.5&	\multirow{3}{*}{59.0}  &\ \ \textbf{59.3}&	84.2 \\
          & \ztree & & \ \ 99.7 &	83.6	& & \ \ 99.9	&84.1	& & \ \ 71.3	&84.1\\
          & \zseq && \ \ 32.8 &	85.1 &&  \ \ \textbf{37.1} &	83.8 &&	\ \ \textbf{59.3}	 &84.1\\
         \midrule
         \multirow{4}{*}{AG News} & None & --- & \ \ 99.9 &	94.5 &---&\ \	99.7	&94.3	&---& \ \ 99.8	& 94.4\\
         \cmidrule{2-11}
         &\ztoken & \multirow{3}{*}{0.6} & \ \ \ \ \textbf{0.6} &	94.4 & \multirow{3}{*}{0.7} &	\ \ \ \ \textbf{0.5}&  94.4	&\multirow{3}{*}{4.1} &  \ \ \textbf{99.1}&	94.2 \\
          & \ztree & & \ \ 99.9 &	94.1 &&	\ \ 99.7	&94.4	&& \ \ 99.6	& 94.3\\
          & \zseq  && \ \ \ \ 0.7 &	94.2 &&	\ \ \ \  0.7	& 94.4	&& \ \ 99.5& 	93.9\\
          \midrule
          \multirow{3}{*}{QNLI} & None &--- & 100.0 &	91.2&--- &	100.0&	91.0&--- &	\ \  99.1	& 89.9\\
          \cmidrule{2-11}
          &\ztoken &\multirow{3}{*}{5.4}  & \ \ \ \ \textbf{4.8} &	91.2& \multirow{3}{*}{4.2} &	\ \ \ \ \textbf{4.6}	& 91.0	& \multirow{3}{*}{3.9} & \ \ 19.6&	90.1 \\
          & \ztree && 100.0	 & 90.7 &&	\ \ 98.8	&91.2	&& \ \ 87.2	& 89.9 \\
          & \zseq && \ \ \ \ 5.6	& 90.4	&& \ \ \ \ 5.2 &	91.1 &&	\ \ \textbf{19.1}	& 90.1\\
         \bottomrule
           
        \end{tabular}
        %}
    \caption{Defence performance of different filtering approaches using z-scores under all attack methods. We \textbf{bold} the best defence numbers across three defensive approaches. \textbf{BASR} indicates the ASR of the benign model over the poisoned test data, which is the lower bound. \textbf{None} means the performance of the compromised models on the poisoned test data, which is the higher bound. The results are an average of three independent runs. For SST-2 and OLID, the standard deviation of ASR and CACC is within 1.5\% and 0.5\%. For AG News and QNLI, the standard deviation of ASR and CACC is within 1.0\% and 0.5\%}
    \label{tab:z-defence}
    % \vspace{-0.5cm}
\end{table*}

% \begin{table}
%     \centering
%     %\scalebox{0.9}{
%     \small
%     \begin{tabular}{clccc}
%     \toprule
%         \multirow{2}{*}{\makecell{\textbf{Attack}\\\textbf{Method}}} &  \multirow{2}{*}{\textbf{Defence}} & \multicolumn{3}{c}{\textbf{SST-2}} \\
%          & & \textbf{BASR} &  \textbf{ASR} & \textbf{CACC} \\
%           \midrule
%         %   \multirow{3}{*}{Benign}& \ztoken\\
%         %   & \ztree\\
%         %   & \zseq\\
%         %   \midrule
%          \multirow{3}{*}{BadNet}& \ztoken &\multirow{3}{*}{9.0}  & \quad 9.4 & 92.3\\
%           & \ztree &  & 100.0  & 92.2\\
%           & \zseq & & \quad \textbf{9.0} & 92.0\\
%          \midrule
%          \multirow{3}{*}{InsertSent} &\ztoken & \multirow{3}{*}{2.9}  &\quad \textbf{3.0} & 92.5\\
%           & \ztree & & 100.0 & 92.5\\
%           & \zseq &  &\quad 3.4 & 92.6\\
%          \midrule
%          \multirow{3}{*}{Syntactic}& \ztoken & \multirow{3}{*}{16.9}& \ \ 37.3 & 91.6\\
%           & \ztree &  &\ \ 29.7 & 92.1\\
%           & \zseq && \ \ \textbf{29.7} & 92.1\\
%          \bottomrule
           
%         \end{tabular}
%         %}
%     \caption{Defence performance of different filtering approaches using z-scores under all attack methods. We \textbf{bold} the best defence numbers across three defence avenues. \textbf{BASR} indicates the ASR of the benign model over the poisoned data without any defence.}
%     \label{tab:z-defence}
%     \vspace{-0.5cm}
% \end{table}

==> tab-ratio-zdefence.tex <==
\begin{table}[t!]
    \centering
    % \scalebox{0.7}{
        \small
    \begin{tabular}{ccrrrrrr}
    \toprule
        \multirow{2}{*}{\textbf{Dataset}} &  \multirow{2}{*}{\makecell{\textbf{Attack}\\\textbf{Method}}} & \multicolumn{2}{c}{\textbf{\ztoken}}& \multicolumn{2}{c}{\textbf{\ztree}}& \multicolumn{2}{c}{\textbf{\zseq}}\\
         & &  \textbf{FRR} & \textbf{FAR} & \textbf{FRR} & \textbf{FAR} & \textbf{FRR} & \textbf{FAR}\\
         \midrule
          \multirow{3}{*}{SST-2} & BadNet &  0.0& \textbf{0.0} & 16.7 & 67.4   & 16.7 & \textbf{0.0}\\
               & InsertSent & 	24.6	& \textbf{0.0} & 23.6 & 0.5 & 25.3&	\textbf{0.0}\\
               & Syntactic & 26.5 & 1.2 & 25.0 & \textbf{0.5} & 26.5 & 1.2\\
               \midrule
              \multirow{3}{*}{OLID} & BadNet &  0.0 &  \textbf{0.0} & 15.4 & 84.0 & 15.5 &\textbf{0.0}\\
               & InsertSent &  3.9 & \textbf{0.0} &	29.1 & 11.9 & 29.1 & \textbf{0.0}\\
               & Syntactic &  1.1 & \textbf{1.2} & 24.1 & 3.9 & 24.1 & \textbf{1.2}\\
                \midrule
           \multirow{3}{*}{AG News} & BadNet &  	3.6	 & \textbf{0.0} &37.6 & 62.9 & 37.6 & \textbf{0.0}\\
               & InsertSent & 5.5 & \textbf{0.0} & 16.6 & 13.6 & 16.6 & \textbf{0.0}\\
               & Syntactic & 12.1 & 	25.9 & 7.3 & 8.0 & 32.1 & 7.2\\
               \midrule
            \multirow{3}{*}{QNLI} & BadNet & \textbf{0.0} & 22.4 & 49.4 & 22.4 & \textbf{0.0}\\
               & InsertSent &  0.3 & \textbf{0.0} & 3.2 & 9.2 & 3.5	& \textbf{0.0} \\
               & Syntactic & 2.9 & 0.5 &10.0 & 10.6 & 10.2  & \textbf{0.5}\\
           \bottomrule
    \end{tabular}
    % }
    \caption{FRR (false rejection rate) and FAR (false acceptance rate) of different z-defences on multiple attack methods. Comparing the defence methods, the lowest FAR score on each attack is \textbf{bold}.}
    \label{tab:detect_z}
    % \vspace{-0.4cm}
\end{table}

